Program Structure Aware Precondition Generation

We introduce a novel approach for inferring natural preconditions from code. Our technique produces preconditions of high quality in terms of both correctness (modulo a test generator) and naturalness. Prior works generate preconditions from scratch through combinations of boolean predicates, but fall short in readability and ease of comprehension. Our innovation lies in, instead, leveraging the structure of a target method as a seed to infer a precondition through program transformations. Our evaluation shows that humans can more easily reason over preconditions inferred using our approach. Lastly, we instantiate our technique into a framework which can be applied at scale. We present a dataset of ~18k Java (method, precondition) pairs obtained by applying our framework to 87 real-world projects. We use this dataset to both evaluate our approach and draw useful insights for future research in precondition inference.

==> 8_future_work.tex <==
\section{Future Work}
\label{sec:future_work}

There are many directions of future work. Firstly, the naturalness of our preconditions as well as the brittleness of the techniques hints toward a statistical method to infer preconditions. \textcolor{red}{cite lots of things that use ML because PL tools dont work at scale.} 

Secondly, there is room to explore the inlining. 

==> algorithms/check.tex <==
\begin{algorithm}
    \caption{Checking function (needs a better name)}\label{alg:check}
    \begin{flushleft}
        \hspace*{\algorithmicindent} \textbf{Input:} Method $M \in \domain{P}$, Precondition $S \in \domain{S}$,
            Environment $I \in \domain{E}$ \\
        \hspace*{\algorithmicindent} \textbf{Output:} Whether $M$ crashing on $I$ indicates a bug
    \end{flushleft}
    \begin{algorithmic}[1]
        \Procedure{check}{$M, S, I$}
        \If{$M(I) crashes$}
            \State \Return \false{}
            \ElsIf{$S(I) = \true{}$}
            \State \Return \false{}
            \Else
            \State \Return \true{}
        \EndIf
        \EndProcedure 
    \end{algorithmic}
\end{algorithm}

==> code_highlight.tex <==
\makeatletter
\newenvironment{btHighlight}[1][]
{\begingroup\tikzset{bt@Highlight@par/.style={#1}}\begin{lrbox}{\@tempboxa}}
	{\end{lrbox}\bt@HL@box[bt@Highlight@par]{\@tempboxa}\endgroup}

\newcommand\btHL[1][]{%
	\begin{btHighlight}[#1]\bgroup\aftergroup\bt@HL@endenv%
	}
	\def\bt@HL@endenv{%
	\end{btHighlight}%   
	\egroup
}
\newcommand{\bt@HL@box}[2][]{%
	\tikz[#1]{%
		\pgfpathrectangle{\pgfpoint{1pt}{0pt}}{\pgfpoint{\wd #2}{\ht #2}}%
		\pgfusepath{use as bounding box}%
		\node[anchor=base west, fill=orange!25,outer sep=.5pt,inner xsep=0.5pt, inner ysep=-0.3pt, rounded corners=2pt, minimum height=\ht\strutbox-.1pt,#1]{\raisebox{.01pt}{\strut}\strut\usebox{#2}};
	}%
}
\makeatother

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}

\lstdefinelanguage{Java}{
  keywords={typeof, new, true, false, catch, function, return, null, catch, switch, var, if, in, while, do, else, case, break, try},
  keywordstyle=\color{blue}\bfseries,
  ndkeywords={class, export, boolean, throw, implements, import, this},
  ndkeywordstyle=\color{darkgray}\bfseries,
  %numbers=left,
  identifierstyle=\color{black},
  sensitive=false,
  comment=[l]{//},
  morecomment=[s]{/*}{*/},
  commentstyle=\color{red}\ttfamily,
  stringstyle=\color{purple}\ttfamily,
  morestring=[b]',
  morestring=[b]"
}

\lstdefinestyle{mystyle}{
% 	backgroundcolor=\color{backcolour}, 
	frame=single,  
	commentstyle=\color{codegreen},
	keywordstyle=\color{blue}\bfseries,
	numberstyle=\tiny\color{codegray},
	stringstyle=\color{codepurple},
	basicstyle=\linespread{0.75}\fontsize{5.8}{9.3}\ttfamily\bfseries,
	breakatwhitespace=false,         
	breaklines=false,                 
	captionpos=b,                    
	keepspaces=true,                 
 	%numbers=left,                    
	numbersep=0pt,                  
	showspaces=false,                
	showstringspaces=false,
	showtabs=false,                
	tabsize=2,
% 	language=[Sharp]C,
	language=Java,
	moredelim=**[is][\btHL]{`}{`},
	moredelim=**[is][{\btHL[fill=red!40]}]{!!!}{!!!},%,draw=red,dashed,thick
	moredelim=**[is][{\btHL[fill=green!40]}]{@}{@},%,draw=red,dashed,thick
}


\lstdefinestyle{mystyle_lineno}{
% 	backgroundcolor=\color{backcolour}, 
	frame=single,  
	commentstyle=\color{codegreen},
	keywordstyle=\color{blue}\bfseries,
	numberstyle=\tiny\color{codegray},
	stringstyle=\color{codepurple},
	basicstyle=\linespread{0.75}\fontsize{5.8}{9.3}\ttfamily\bfseries,
	breakatwhitespace=false,         
	breaklines=false,                 
	captionpos=b,                    
	keepspaces=true,                 
 	numbers=left,                    
	numbersep=-3.5pt,                  
	showspaces=false,                
	showstringspaces=false,
	showtabs=false,                
	tabsize=2,
% 	language=[Sharp]C,
	language=Java,
	moredelim=**[is][\btHL]{`}{`},
	moredelim=**[is][{\btHL[fill=red!40]}]{!!!}{!!!},%,draw=red,dashed,thick
	moredelim=**[is][{\btHL[fill=green!40]}]{@}{@},%,draw=red,dashed,thick
}




==> old_submission/4_technique.tex <==
\section{Technique}
\label{sec:technique}
In this section, we address the second challenge: learning a precondition synthesis function $G : \domain{P} \rightarrow \domain{S}$. 
To do so, we experiment with two approaches. The first, is a generative transformer model finetuned on our dataset of (MUT, precondition) pairs. The second approach includes an intent detection backbone model, to condition generation of the precondition.

\subsection{Generative Transformer Model}
To learn $G$, we finetune a generative model of code, CodeT5~\cite{CodeT5}. In contrast to GPT~\cite{GPT2, GPT3, Codex} (decoder only) models or BERT~\cite{BERT, codebert} (encoder only) models, T5~\cite{T5} is an encoder-decoder framework, making it ideal for translation or other seq2seq tasks. CodeT5 is a programming language model which represents code as a sequence of tokens. It is pretrained on masked language modeling with a special identifier aware code pretraining task. We finetune the model using cross entropy loss over our supervised dataset $D_1 = ((M*,S)_1, ..., (M*,S)_n)$ where $M*$ is a correct MUT and $S$ is the generated precondition label. 

\subsection{Intent Query + Generative Transformer Model}
An alternate approach we propose is a two-stage technique consisting of an intent query backbone and a generative model. \textit{Intent detection} is a crucial mechanism in speech recognition~\cite{SLU, joint-intent}, natural language understanding~\cite{bert-intent}, and dialog systems such as chat bots~\cite{dialog-intent}. Intent detection is a classification problem over a set of semantic intents. For example, ATIS~\cite{ATIS} (Airline Travel Information System) is a dataset of (text, intent) pairs. Given an input: \textit{"Please find a flight from St. Petersburg to Miami on Thursday"}, the intent is a label of the semantic meaning: \textit{find flight}. A single input may also have multiple intents: \textit{"list all Sunday flights from Cleveland to Nashville and their fares"} => \textit{find flight + airfare}.  Such an intent classification system can aid in downstream generative tasks. They lighten the burden on generative models which otherwise must be able to discern the input intent along with generating an appropriate response.

In the setting of precondition inference, we abstract the intentions of a method's designer into 7 distinct categories of checks:
\begin{itemize}
    \item \code{npe}: Check for Null Pointer Exceptions
    \item \code{explicit}: Check for explicitly thrown exceptions
    \item \code{call}: Check for exceptions possibly thrown by callees within the method
    \item \code{negArray}: Check for arrays initialized with negative numbers
    \item \code{aob}: Check for array accesses which may be out of bounds
    \item \code{cast}: Check for incorrect object casts
    \item \code{arith}: Check for errors in arithmetic expressions
\end{itemize}

Each method may have a set of zero or more associated intents.
We therefore frame the intent prediction problem as a binary querying task.
%Assume that $\domain{P}$ denotes the set of all methods, and $\domain{Intents}$ denotes the set of all intents.
We aim learn to function: $G_{intent}$ with produces a binary label given an input MUT and intent type. The single function is capable of classifying over all 7 intent types. To learn such a function $G_{intent}$, we finetune CodeT5's encoder over a supervised dataset:
$D_2 = ((M*, It, B)_1, ..., (M*, It, B)_n)$, where $M*$ is a correct method, $It$ is an intent, and $B \in \code{Bool}$ is \true{} iff $M*$ has intent $It$. 
Recall CodeT5 is an encoder-decoder transformer architecture trained end to end with cross entropy loss. For a querying classification task, only an encoder is necessary.

The Intent Query Model at inference time is shown in Figure~\ref{fig:intent-model}. For a single MUT, 7 calls are made to $G_{intent}$. From the binary predictions, a set of intents, $M_{intent}$, is collected such that:
$\forall In \in M_{intent}, G_{intent}(M, In) = \true$.

\begin{figure}[]
    %\begin{subfigure}[b]{0.4\linewidth}
    \includegraphics[width=.3\textwidth]{artifacts/intent-query-model.pdf}
    \caption{Intent Query Model.}
	\label{fig:intent-model}
    %\end{subfigure} 
\end{figure}


\subsubsection{Stage 2: Intent-driven Precondition Synthesis}
%Once our intent model has obtained $M_{intent}$, w
Our next stage utilizes the intent set obtained in Stage 1 through prompt-based learning. Prompt-based learning~\cite{prompt-learning}, is a paradigm in which pretrained language models are adapted to downstream tasks through a textual prompt. Consider a machine translation task which translates French to English. In the traditional supervised learning paradigm, a model would be trained on a dataset of (French, English) pairs with the French 
phrase being the input to the model and the English as the output. In contrast, translation as prompt based learning is formulated with the input to the model including a description of the task:

\noindent \textbf{French}: \textit{Je vous aime.} \\
\textbf{English}: \\

Such an input formulates the task as autocomplete. Prompt based learning has advantages in that it assists the model by explicitly defining the task in the input. 

We formulate precondition synthesis as prompt-based learning with a \textit{prefix} intent prompt as shown in Figure~\ref{fig:gen-model}. The prompt format is the following: 
\\
\noindent \textbf{\#\# $M_{intent}$ \#\# $M$}  \\
Again, we finetune CodeT5 with cross entropy loss to synthesize preconditions. However, in this approach we train with a dataset $D_3 = ((\#\# M_{intent} \#\# M*, S)_1, ..., (\#\# M_{intent} \#\# M*, S)_n)$ where $M*$ and $S$ are correct methods and precondition labels in our dataset.
%\TODO{TIE IN THEE OTHER DIAGRAM}
%given the method $M$ and the set of its corresponding intents $M_{intents}$,
%by learning a function $G_{synth}: \domain{P}, \domain{I} \rightarrow \domain{S}$.
%We do so over the training set $(M, M_{intents}, S)$....

\begin{figure}[]
    \includegraphics[width=.3\textwidth]{artifacts/gen-model.pdf}
    \caption{Generative Model Conditioned on Intent.}
	\label{fig:gen-model}
\end{figure}




==> old_submission/old_1.5_related.tex <==
\section{Related Work}
\label{sec:related}

In this section, we outline prior approaches to precondition synthesis. Prior approaches include {\it static}, {\it dynamic} and natural language processing ({\it NLP}) based techniques.

\subsection{Static approaches}

Houdini~\cite{houdini-esc} uses a fix-point computation to infer the strongest precondition over a set of predicates using a modular verifier.
Abductive approaches~\cite{das-cav15,Albarghouthi-popl16} infer environment specifications (including preconditions) that are sufficient to verify assertions in a method.
SnuggleBug~\cite{snugglebug-pldi2009} uses backward propagation of weakest precondition to synthesize invariants.
Alur et al.~\cite{alur-popl05} synthesize interface specifications of classes using predicate abstraction based model checking. 
The symbolic approaches often do not scale to real-world programs  due to the need to come up with a small class of predicates to express preconditions, or suffer from loss of precision in the presence of loops, nested procedures and complex frameworks.
By posing the precondition inference problem as an executable code generation task, our framework is expressive and does not require a small set of predicates. 
However, unlike these approaches, we fail to provide any guarantees of soundness about the preconditions constructed using our technique, and resort to empirical guarantees such as accuracy on a large dataset. 

%1) Houdini - uses a guess and check approach with the ESC checker 
%2) SnuggleBug - does backwards propogation of weakest preconditions but struggles where you would expect (scaling in the presence of loops, aliasing, virtual method calls...)
%3) temporal precondition inference (don't infer a formal spec but instead say A must be called before B)... // interface Alur
%5) necessary preconditions - cousot, francesco 
%6) angelic verification
%7) maximal specification synth

%Does not work on dynamic, frameworks, need predicates, ....

\subsection{Dynamic approaches}
Dynamic approaches infer invariants based on generalizing concrete values obtained during testing over a set of templates.
Daikon~\cite{daikon} infers relationships between program variables and can synthesize candidate invariants.
However Daikon's invariants can be too strong given the limited number of tests (e.g., stating that a parameter equals 0), as observed in prior works~\cite{are-my-invariants-valid}.
Sankaranarayanan et al.~\cite{Sankaranarayanan-issta08} uses decision-tree classifier learning to create precondition over a Boolean combination of a set of predicates. 
Padhi et al.~\cite{Padhi-pldi16} uses program synthesis over a grammar to infer predicates needed to synthesize preconditions over runtime traces.
Unlike these approaches, our formulation of precondition as a program is not restricted by the need for a grammar, and thus more expressive. 
Moreover, our neural synthesis is scalable without the need for searching over the exponential space defined by the predicates. 

%There are also existing approaches for invariant detection. This could maybe be adapted to preconditions by putting it at the beginning of the method?
%1) Daikon -- conjunction
%2) Sankarayan et al. -- boolean combination of predicates 
%3) data-driven precondition -- infer the predicates 
%We do more expressive because we construct a program taking subparts of programs, and also scalable. But it is not declarative. 

\subsection{NLP and ML based methods}

Finally, there have been approaches to synthesize preconditions directly from the comments and docstrings present on a method. 
JDoctor~\cite{JDoctor} generates executable preconditions by rule-based natural language processing of the JavaDoc comments. 
Similarly, C2S~\cite{c2s} translates JavaDoc comments to formal specifications in Java Modeling Language using syntax-guided synthesis and test-guided pruning.
TOGA~\cite{TOGA} synthesizes exceptional test oracles for test cases using a neural approach.
Unlike these approaches, our method does not require the presence of a rich descriptive comment to synthesize the precondition.
However, combining our approach with precondition templates generated from comments is an important avenue for future work. 

%1) Toradocu / Jdoctor --> heuristics based on tokens, 
%3) Swamy - ECMA script template specs -> precondition (doesn't apply to general comments)
%Both rely on comments/docstring
%3) TOGA - ??


%----

%\subsection{Methods for Postcondition Inference}
%There's also works for post condition inference like....
%1) EvoSpex / EvoSuite assertion learning..
%2) ATLAS / neural assertion generation


%\subsection{Methods for Test Oracle Inference} 
%Test oracle inference is given a prefix, what should the behavior be? This is a generalization of pre/post condition inference. 



%1) TOGA - does assertions but also can be adapted to precondition inference if you consider any "intended" exception as a precondition violation
%2) JDoctor / Toradocu


%contract inference?


==> old_submission/old_2_problem_setup.tex <==
\section{Problem Setup}
\label{sec:setup}
In this section, we formalize the problem of precondition inference as a code generation task and relate it to existing approaches.
%% In other words, C is a perfect classifier for legal vs illegal for correct methods
% Think about JIST, considering that the tools assume that the method is correct
% define C
Let $\domain{P}$ denote the set of all executable methods, and $\domain{E}$ denote the set of all program
environments. Let $M$ denote any method in $\domain{P}$, and $M*$ denote any method that is \emph{correct}.
Let $I$ denote any environment in $\domain{E}$.

Consider a function $C: \domain{P}, \domain{E} \rightarrow \code{Bool},$ such that $C(M, I) = \true$ if
and only if $M$ exits normally on environment $I$ without crashing. On a correct method $M*$, $C(M*, I) = \true$ if and only if $I$ is a legal environment of $M*$. In other words, $C$ is a perfect classifier for the legality of any $I$ given a correct method $M*$. Note that $C$ is a realizable function, so long as $M*$ is executable.


We define the ideal precondition as the function $\sIdeal : \domain{P}, \domain{E} \rightarrow \code{Bool}$,
such that $\sIdeal(M, I) = \true$ if and only if $I$ is a legal environment of $M$.
Moreover, since $C$ can perfectly classify $I$ for any correct $M*$, we note that
\begin{equation}
    \sIdeal(M*, I) = C(M*, I)
\end{equation}
Since $C$ is realizable, $\sIdeal$ is also realizable for correct methods.
However, for methods whose correctness may not be known, such an ideal precondition is not realizable.
In these cases, different tools will attempt to approximate $\sIdeal$ using a variety of techniques.

% define S
% For a particular method M,
% S: E -> Bool, S(I) = true for illegal environments wrt M, and false for legal environments wrt M.

% Define C: P, E -> Bool, such that C(M, I) = true iff M crashes on I
% Note: C(M*, I) = false on legal environments

% add M in a subscript

% Let $\domain{P}$ denote the set of all executable methods, and $\domain{E}$ denote the set of all program
% environments.
% For a particular method $M \in \domain{P}$, we define a precondition as the function
% $S : \domain{P}, \domain{E} \rightarrow \code{Bool}.$
% % which returns \true{} for illegal inputs and \false{} for expected ones.

% In order to define $S$, we also define the function $C: \domain{P}, \domain{E} \rightarrow \code{Bool},$
% such that for any $M \in \domain{P}$ and $I \in \domain{E}$, $C(M, I) = \true$
% if and only if $M$ crashes when run with environment $I$, and false otherwise.
% % \begin{align}
% %     \forall M \in \domain{P}, I \in \domain{E}, C(M, I) =
% %         \begin{cases}
% %             \true & \text{if $M$ crashes on $I$} \\
% %             \false & \text{otherwise}
% %         \end{cases}
% %     \label{eqn:exec_definition}
% % \end{align}
% Note that for any \emph{correct} method $M* \in \domain{P}$, and any environment $I \in \domain{E}$,
% % $C(M, I) = \false$ for all \emph{legal} environments $I$, and $C(M, I) = \true$ for all \emph{illegal} environments $I$.
% \begin{align}
%     C(M*, I) =
%         \begin{cases}
%             \true & \text{if $I$ is illegal for $M*$} \\
%             \false & \text{otherwise}
%         \end{cases}
%     \label{eqn:exec_correct}
% \end{align}

% % -- Ideal precondition
% % S_ideal(I) is unrealizable, but we know S_ideal(I) for all correct methods M*
% % because C(M*, I) = S_ideal(I).

% Let $\sIdeal$ denote the ideal precondition.
% For a given method $M \in \domain{P}$,
% $\sIdeal$ for $M$ exhibits the following behavior:
% \begin{align}
%     \sIdeal{}(M, I) =
%         \begin{cases}
%             \true & \text{if $I$ is illegal for $M$} \\
%             \false & \text{otherwise}
%         \end{cases}
%     \label{eqn:ideal_precondition}
% \end{align}

% Such an ideal precondition is unrealizable for most methods.
% However, for \emph{correct} methods, the ideal precondition can be expressed in terms of $C$.
% From Equations \ref{eqn:exec_correct} and \ref{eqn:ideal_precondition}, we can infer that for a
% particular correct method $M* \in \domain{P}$:
% \begin{align}
% \sIdeal(M*, I) = C(M*, I)
% \end{align}

% However, when the correctness of a method is not known, various tools attempt to approximate $\sIdeal$
% using different techniques.

% -- Randoop's precondition:
% Randoop uses a fixed set of flags to implement S_Randoop
For instance, \randoop{} uses a fixed set of flags to define its precondition $\sTool{\randoop}(M, I)$, independent of the input method $M$.
% The following quote was taken from Randoop's manual.
We quote the Randoop manual in \autoref{fig:randoop_manual}.

\begin{figure}
    \framebox{%
        \begin{minipage}{\linewidth}
            By default, a thrown exception is not considered to indicate an error in the code under test. This is because a method may have a precondition that is unknown to Randoop. For example, a binary search implementation might require that its input is sorted. Randoop should not mark the method as buggy just because it throws an exception when Randoop passes it an ill-formed unsorted array. \textbf{Randoop has no way of knowing each method's precondition. In order to avoid outputting an "error-revealing test" that doesn't reveal an error but merely misuses the software under test, by default Randoop assumes that any exception thrown by a method is correct behavior in response to the values that it was passed.} \\ \\
            Checked exceptions: \textbf{default: expected} \\
            NullPointerException when null is passed as an argument to any method in the test. \textbf{default: expected} \\
            NullPointerException when only non-null values are provided as an argument. \textbf{default: invalid} \\
            Unchecked exceptions other than NullPointerException, including AssertionError. \textbf{default: expected}
        \end{minipage}
    }
    \caption{Randoop's heuristics as specified in its manual.}
    \label{fig:randoop_manual}
\end{figure}

% -- TOGA's precondition:
% S_TOGA is a function which makes a call to a large language model TOGA: P, E --> Bool
% such that TOGA(M, I) is trained to return true if I is *likely* an illegal environment wrt M.
\toga{} \cite{TOGA} defines $\sTool{\toga}(M, I)$ as a function which calls a large language model classifier.
%$\toga: \domain{P}, \domain{E} \rightarrow \code{Bool}$.  
TOGA is trained on developer written tests to classify exceptions as expected or unexpected. In other words, TOGA outputs a binary label that represents if $I$ is likely an illegal environment for $M$.


% -- JDoctor's precondition
% JDoctor defines S_JDoctor by translating docstrings into a set of preconditions via a set of predetermined
% natural language heuristics, such that S_JDoctor returns true if it believes that the natural language
% docstring specifies that I is an illegal environment
\jdoc{} \cite{toradocu} defines $\sTool{\jdoc}$ by translating docstrings into precondition predicates using a set of predetermined natural language templates. For example, the keywords ``\texttt{is/are positive}'' translates to ``\texttt{> 0}'' in the predicate. $\sTool{\jdoc}$ evaluates the predicates during testing and returns a boolean indicating if the constructed precondition is satisfied.
%, such that for any $\sTool{\jdoc}(M, I) = \false$ if the heuristics determine
%that the natural language docstring specifies that $I$ is an illegal environment.

% -- Our Approach
% Goal: Formulate the problem of inferring S as a code gen problem.
% Therefore the goal is to synthesize precondition program S, given Method M and environment I
% define function gen to generate S
In contrast, we formulate the problem of inferring $S$ as a code generation problem.
Let the set $\domain{S} \subseteq \domain{P}$ denote the set of all the precondition programs.
We construct a function $G : \domain{P} \rightarrow \domain{S}$ to synthesize a precondition program $\sTool{\toolName}$
given some $M$.
Our goal is, therefore, to learn the function $G$ such that $\sTool{\toolName}$ approximates $\sIdeal$ as closely as possible.
The definition of $G$ can be learned by training a neural model over a dataset of pairs of
$(M*, S) \in \domain{P} \times \domain{S}$, where $M*$ is a \emph{correct} method, and $S$ is its minimal executable precondition.

% Strengths
% Answer
% -- Why choose executbale preconditions instead of predicates (expressiveness)
%    -- can't wrap callees into try-catch blocks
% -- Why do executable preconditions instead of classification (vs TOGA, portability, interpretable)

% This effectively represents the problem of inferring precondtion as a code generation problem.
Formulating precondition inference as a code generation problem has several advantages over alternate approaches. Preconditions represented as executable programs are:
\begin{enumerate}
    \item \textbf{Expressive.}
        Executable programs are inherently more expressive than predicates or flags.
        %Our problem setup represents preconditions as executable programs, which are inherently more expressive
        %than representations such as predicates or flags.
        Treating preconditions as programs allows for guarding against specific errors, like illegal typecasts and
        exceptions thrown by callees.
        For example, consider \autoref{fig:mut_example}. Function \code{opName}'s precondition, as shown
        in \autoref{fig:pre_mut_nested_call}, requires wrapping a call to \code{next(1)} in a \code{try-catch}
        block. Representing the precondition: ``If \texttt{next(1)} throws an exception, $I$ is illegal'' is not possible
        with a predicate.
    \item \textbf{Interpretable.}
        Representing preconditions as programs rather than black box classification, allows for interpretability. 
        A developer can examine the generated code to ensure that the precondition is correct on a wide variety of inputs.
        Moreover, the developer can edit the precondition to their liking, and commit it for use in further testing.
    \item \textbf{Portable.}
        The executability of the generated preconditions ensures that they are portable, meaning that they can
        be used with any testing tool by integrating the preconditions into the test drivers generated for that
        method.
        %On the other hand, tools like \toga{} are trained over environments generated by specific
        %testing tools that cannot be generalized to other tools, and porting the exception oracle used by
        %\randoop{} for use in other tools would require heavy engineering efforts.
\end{enumerate}

In order to realize $\sTool{\toolName}$, we must address two significant challenges:
\begin{enumerate}
    \item \textbf{Generating the Dataset.}
        It is difficult to obtain ground-truth preconditions, as they are rarely formally written in practice.
        Furthermore, they cannot be generated for an $M$ that is not known to be correct as $\sIdeal$ is unrealizable. 
        Generating a dataset $D \subset \domain{P} \times \domain{S}$ over which $G$ can be learned is challenging.
        To generate such a dataset, we exploit the property that $\sIdeal$ is realizable for correct methods. 
        This allows us to mine trustworthy projects for methods and generate their preconditions by observing $C$.
        We elaborate on the dataset generation in more detail in \autoref{sec:dataset}.
    \item \textbf{Learning the precondition synthesis function $G$.}
        Once a high-quality dataset is generated, learning $G$ is still a challenge.
        This arises primarily from the fact that $G$ is now a code generation function, which must synthesize the
        executable precondition given $M$.
        While contemporary methods do so by assuming $M$ to be correct, our problem setting makes no such assumption.
        Therefore, $G$ must learn to distinguish between the components of $M$ that may divulge the intent of the
        developer, and the components that may potentially contain bugs.
        We therefore frame $G$ as an intent-driven code generation system. It first isolates the intent
        of the developer by deciding the checks that need to be included in the precondition, then takes
        this intent into account while synthesizing the precondition itself.
        We elaborate on our technique in \autoref{sec:technique}.
\end{enumerate}

% no documentability


==> old_submission/old_3_dataset.tex <==
\section{Dataset}
\label{sec:dataset}

Constructing a large scale dataset of preconditions, or program specifications of any kind, is a challenge as they are rarely written in practice. Previous approaches have attempted to create such a dataset. In C2S~\cite{c2s}, the authors collect developer written JML specifications from the JDK. The resulting dataset contains 3,547 specifications which is too small for machine learning techniques and leads to overfitting. 

Another approach~\cite{are-my-invariants-valid} avoids the need for developer written specifications by generating specifications from the program behavior using Daikon~\cite{daikon}. Daikon uses program traces to report properties that were true across all executions. Unfortunately, Daikon suffers from incompleteness and often fails to generate a representative set of program executions. The authors also found that Daikon's invariants are often unhelpful and report obvious or uninteresting invariants. Although works exist to statically generate a symbolic specification~\cite{snugglebug}, generating a large scale dataset is infeasible in the presence of loops, nested procedures, dynamic typing and other constructs common in real world code. Another static approach~\cite{bodyguard} attempts to generate a dataset of invariants. The authors do this by considering an if-statement's guard condition to be an invariant of the guarded block. Although they were able to collect these invariants on a large scale (2.5 million invariants), such a dataset cannot capture implicit specifications that are not expressed directly in \texttt{if} conditions. 

Lastly, an approach~\cite{crowdsource-preconditions} attempts to crowdsource preconditions abstractly. The crowdsourcing only yielded a few hundred preconditions, many of them bad quality. Furthermore, such an approach requires manual effort and would be difficult to scale.

\subsection{Dataset Generation}

We take a new approach to generating a large-scale dataset of preconditions by exploiting the property that $S_{ideal}$ is realizable for correct methods. As a proxy for correct methods, we collect a set of popular, stable, high quality Java projects. Because they are highly used and tested, we make the assumption that all methods in the training set are correct. With this assumption, we can construct $S_{ideal}$ based on the behavior of $C$. That is, if a correct method under input $I$ crashes, $I$ is an illegal environment. 

In order to realize $S_{ideal}$ through $C$, two components are needed. First, we need an oracle of exceptional behavior: $O$. The oracle must 
be an exhaustive enumerator of environments. Second, we require a \textit{slicing} mechanism to identify program segments which are related to exceptional behavior. % We employ a program reducer, Perses~\cite{perses}. 

At a high level our data generation process (Algorithm ~\ref{alg:data_gen}) is as follows:
We begin with the method under test and transform it into a \textit{precondition template} by making small modifications to conform to the signature of $S$ defined in section~\ref{sec:setup}. Next, we use a regression test generator, EvoSuite~\cite{EvoSuite}, to generate an exceptional behavior oracle $O$. Lastly, we use a program reducer with the EvoSuite generated tests as an oracle to remove program segments that are unrelated to the exceptional behavior. Assuming the method under test is correct and the test generator is exhaustive, this process results in an $S_{ideal}$.


%Algorithm 1:
%Perhaps use generic term instead of evosuite, e.g. generateRegressionTests.
%handleImplicitExceptions should take another argument, otherwise it is not clear what is causing it to return a new S each time it is called.  Maybe execSuite returns something which is then passed to it.  In that case, perhaps use a more descriptive name, e.g. findImplicitExceptions.
%I don't know why you run the test suite again in the body of the loop; how can O change if S is only modified to handle implicit exceptions?

%\TODO{FIX THE FOLLOWING -> (1) S someimes not italics (2) C\_suite is not defined (3) handleImplicitExceptions need to take the output of C}

\begin{algorithm}
\caption{\label{alg:data_gen} Data Generation}
\begin{algorithmic}[1]
\Procedure{genPrecondition}{M}
\State $S_{init} \gets \texttt{createPreconditionTemplate}(M)$
\State $O \gets \texttt{exceptionalBehaviorOracle}(S_{init})$ 
\State $S \gets S_{init}$
\While{\texttt{stack\_trace} = $RUN(S, O)$}
   \State $S \gets \texttt{handleImplicitExceptions}(S, \texttt{stack\_trace})$
    \State $O \gets \texttt{exceptionalBehaviorOracle}(S)$ 
\EndWhile

\State $S \gets \texttt{reducer}(S, O)$
\State \Return $S$ 
\EndProcedure 
\end{algorithmic}
\end{algorithm}


Our dataset is collected from 130 Java projects. The projects are from the SF100~\cite{EvoSuite-challenges} dataset with 30 additional projects collected from the most popular projects in the Maven Repository.

We will illustrate the MUT to precondition transformation using the \texttt{Stack} constructor in Figure~\ref{fig:stack_m} to obtain its precondition \texttt{Stack\_pre} in Figure~\ref{fig:final_pre_stack}. 

\begin{figure} %[hb]
    \begin{subfigure}[]{.4\linewidth}
    \lstset{style=mystyle, xleftmargin=.0\textwidth, xrightmargin=0.1\textwidth} %, linewidth=0.2\linewidth}
    \lstinputlisting[linewidth=4.3cm]{./examples/Stack_constructor.java}
    \caption{Stack Method Under Test (MUT).}
    \label{fig:stack_m}
    \end{subfigure}
    \begin{subfigure}[]{.4\linewidth}
    \lstset{style=mystyle, xleftmargin=.1\textwidth, xrightmargin=0.0\textwidth} %, linewidth=0.2\linewidth}
    \lstinputlisting[linewidth=4.3cm]{./examples/Stack_template.java}
    \caption{Stack Precondition Template.}
    \label{fig:s_init}
    \end{subfigure}

    \begin{subfigure}[]{.4\linewidth}
    \lstset{style=mystyle, xleftmargin=.0\textwidth, xrightmargin=0.1\textwidth} %, linewidth=0.2\linewidth}
    \lstinputlisting[linewidth=4.3cm]{./examples/Stack_wrapped.java}
    \caption{Precondition with Implicit Exception Wrapped.}
    \label{fig:s_wrapped}
    \end{subfigure}
    \begin{subfigure}[]{.4\linewidth}
    \lstset{style=mystyle, xleftmargin=.1\textwidth, xrightmargin=0.0\textwidth} %, linewidth=0.2\linewidth}
    \lstinputlisting[linewidth=4.3cm]{./examples/Pre_Stack.java}
    \caption{Final Precondition.}
    \label{fig:final_pre_stack}
    \end{subfigure}
    %\label{fig:pre_stack}
   \caption{Example Data Collection Process, from Method Under Test to Precondition.}
\end{figure} 

\parheader{Precondition Template.}
The first step of dataset collection is to create a precondition template. Such a template is a boolean returning function with the same parameters as the method under test, as defined in Section~\ref{sec:setup}. The body of the precondition template is copied from the method under test. Modifications are made such that the template returns boolean values. Any explicitly thrown exception using the Java \texttt{throws} keyword, is replaced with a ``\texttt{return false;}'' statement. Any non-boolean returning \texttt{return} statements are replaced with ``\texttt{return true;}'' while retaining the original return expression. Lastly, each method invocation is split onto its own line. We explain the reason for separation of nested calls in the Implicit Exception Handler section. A complete precondition template is shown in Figure~\ref{fig:s_init}. 

\parheader{Exceptional Behavior Oracle.} 
In order to construct $S_{ideal}$, we require an oracle of exceptional behavior, $O$. For such an oracle, we use the automated regression test generator, EvoSuite. EvoSuite generates both legal and illegal inputs and reports the behavior (Figure~\ref{fig:stack-evo}). If EvoSuite finds an input which crashes the method under test, we consider it to be illegal. As such, $S_{ideal}$ should return false. Assuming EvoSuite exhaustively covers all input states, we can construct $S_{ideal}$. Since EvoSuite is a dynamic testing tool, it does suffer from incompleteness. However, we conducted a manual study to evaluate our assumption. We inspected 50 MUTs in our training set and manually identified possible crash points. Then, we inspected the Evosuite exceptional behavior oracles to confirm that all identified crash points were indeed executed by EvoSuite. We found that only 8/50 test suites did not find a crash point which we had manually identified.

\begin{figure}[]
    \lstset{style=mystyle, xleftmargin=0.0\textwidth, xrightmargin=0.0\textwidth, linewidth=0.2\linewidth}
    \lstinputlisting[linewidth=8.5cm]{./examples/Stack_ESTest.java}
   \caption{Evosuite Generated Exception Behavior Oracle}
    \label{fig:stack-evo}
\end{figure}

\parheader{Implicit Exception Handler.}
Our precondition should not throw an exception on an illegal input, but instead return false. Given the EvoSuite behavior oracle in Figure~\ref{fig:stack-evo}, our data collection process must modify the precondition so it returns false in \texttt{test1} rather than crashing. Our \textit{Implicit Exception Handler} inserts a check prior to the crash point based on the crash type. We chose the 6 following exception types empirically such that over 99\% of the crashes EvoSuite found during data generation fit these exception types.

\begin{enumerate}
\item \texttt{java.lang.NegativeArraySizeException} \\
$\texttt{...\textbf{new T[i]}...} \rightarrow \texttt{if (\textbf{i} < 0) return false; ...}$

\item \texttt{java.lang.ArrayIndexOutOfBoundsException} \\
$\texttt{...\textbf{a[i]}...} \rightarrow \texttt{if (\textbf{i} < 0 || \textbf{i}  >= \textbf{a}.length) return false;...}$

\item \texttt{java.lang.NullPointerException} \\
$\texttt{...\textbf{a.foo}...} \rightarrow \texttt{if (a == null) return false;...}$

\item \texttt{java.lang.ArithmeticException}\\
$\texttt{...\textbf{a/b}...} \rightarrow \texttt{if (\textbf{b} == 0) return false; ...}$

\item \texttt{java.lang.ClassCastException} \\
$\texttt{...\textbf{(T) a}...} \rightarrow \texttt{if (!\textbf{a} instanceof \textbf{T}) return false; ...}$

\item \texttt{Intraprocedural Exceptions} \\
$\texttt{...bar()...} \rightarrow$ \\ 
$\texttt{try \{ \textbf{bar()} \} except (Exception e) \{ return false; \}...}$
\end{enumerate}

Note that we choose to wrap calls in a try-catch as in Figure~\ref{fig:mut_example}. Rather then including potentially complex precondition logic from the body of the callee, we make the decision to wrap crashing calls in the MUT in try-catch blocks. We do this because the callee may invoke a long chain of calls for which extracting all of the precondition logic would result the precondition being unreadable. It is safe to assume that a crashing call in the MUT is a precondition violation. A callee may crash because of (1) a bug in the callee, (2) a bug in the MUT causing a precondition violation of the callee, or (3) a precondition violation of the MUT. While collecting data, we assume all methods in the project are correct. So, a crash in a callee must be a precondition violation of the MUT.

EvoSuite and the \textit{implicit exception handler} are called in a loop until EvoSuite can no longer find crashing inputs to the precondition.
Such a precondition is shown in Figure~\ref{fig:s_wrapped}

\parheader{Program Reducer.}
Lastly, we invoke a program reducer to remove components of the precondition which are not related to the precondition's return behavior. The preconditions produced are minimal: if any program segment is removed, the behavior (according to EvoSuite) will change. Minimality is desirable in our dataset for interpretability and learnability. For example, Figure~\ref{fig:s_wrapped} shows the precondition prior to reduction while Figure~\ref{fig:final_pre_stack} shows the precondition after reduction. The reduction creates a more desirable precondition.

To reduce the precondition, we use Perses~\cite{perses}, a syntax guided program reducer. Perses takes as input a program to reduce and a set of constraints. Perses outputs the smallest sub-program which satisfies the constraints. In our setting, the constraints are that every EvoSuite regression test must pass. We also experimented with the c-reduce~\cite{c-reduce} reducer but found it to be time-inefficient as it considers syntactically invalid sub-programs which increases the search space.

\subsection{Final Dataset}
We run the data generation process on a high quality set of precompiled Java projects. The projects were collected from the SF100 dataset~\cite{EvoSuite-challenges} plus the 30 most popular projects from the Maven repository.
Our data collection process does not produce a precondition for every input method. Nearly 80\% of MUTs fail to produce an precondition due to compilation errors or EvoSuite failures. On large scale real world code, EvoSuite sometimes struggles to generate test suites due to resource limits, concurrency, and missing environment dependencies~\cite{EvoSuite-challenges}. These challenges prevent our data collection process from reliably producing a precondition at test time. Furthermore, our dataset collection process assumes correct code, rendering it ineffective for bug finding.

In addition to a dataset of (MUT, precondition) pairs, we also construct a dataset of (MUT, exceptional behavior oracle) pairs from the EvoSuite tests. The exceptional behavior oracle produced by EvoSuite, along with its execution environment is a valuable tool for evaluation. Equivalent code may not syntactically match. By testing a predicted precondition with the EvoSuite tests created during dataset collection, we can measure a semantic performance metric. Lastly, we also record the check types added by the implicit exception handler in (MUT, exception type, boolean) pairs where boolean indicates whether the crash type was found in the MUT.

\begin{table}[t]
\resizebox{.4\textwidth}{!}{
{\small
	\begin{tabular}{c|ccc}
	\toprule
        Crash Type                              & Train & Val & Test \\
        \cmidrule(l){1-4}
		Overall                                 & 23,930 & 2,621 & 4,255 \\
        \cmidrule(l){1-4}
		No crash                                & 11,764  & 1,513   & 3,162     \\
		\texttt{NullPointerException}           & 2,162  & 246   & 280     \\
		Explicit \texttt{throw} expression      & 1,516  & 63   & 24     \\
		Intraprocedural Exception               & 4,589  & 433   & 399     \\
		\texttt{NegativeArraySizeException}     &    31  & 0   & 1    \\
		\texttt{ArrayIndexOutOfBoundsException} &    62  & 1   & 4    \\
		\texttt{ClassCastException}             &    18  & 9   & 5   \\
		\texttt{ArithmeticException}            &    1  & 1   & 2    \\
		Multiple Exceptions                     & 3,787 & 355   &  378   \\
	 \bottomrule
	\end{tabular}
    }}
	\caption{Dataset Breakdown by Crash Type}
    \label{tab:data-breakdown}
\end{table}



==> old_submission/old_5_eval.tex <==
\section{Evaluation}
\label{sec:eval}

In this section, we evaluate our approach with the goal of answering the following research questions:

%\parheader{Research Questions.} We consider the following research questions in our evaluation:
\begin{enumerate}
 \item[\textbf{RQ1}] How accurate are the preconditions generated by our approach?
 \item[\textbf{RQ2}] How effective is our approach in conjunction with a randomized testing tool?
 \item[\textbf{RQ3}] How robust is our approach to bugs in the method under test?
\end{enumerate}

%\parheader{Datasets.} Our evaluation uses two datasets. A intent dataset and a generation dataset. We create a train-dev-test split of \TODO{x:y:z}. We ensure that there is no project-level overlap between splits. Our project level split is \TODO{in the appendix}. 

%\parheader{Bug Benchmark.} 
%We evaluate real-world bug finding on the Defects4J~\cite{defects4j} benchmark. Defects4J is a benchmark of 835 bugs from 17 real-world Java projects. Each sample in the benchmark includes both buggy and fixed code versions. Each fixed program version is based on a minimal patch to fix the bug, and passes all the project tests, while each buggy program version fails at least one test. Each bug is based on an error that was logged in the project's issue tracker, involves source code changes, and is reproducible \ie{with a deterministic test}. The benchmark also includes utilities for generating and evaluating test suites on the programs to determine if generated tests pass on the fixed versions and catch bugs. \\


%Because each defects4j "bug" is based on a minimal patch, we consider any test which fails the buggy version and passes the fixed version to be the same bug. Many unique test prefixes may find a same bug.

\subsection{RQ1: Precondition Generation Accuracy} To answer RQ1, we report the performance of the End-to-End system as well as the Intent Query Model in isolation on a held out test set.

\parheader{Dataset.} 
Our evaluation uses three datasets. The first is a dataset of intents. The dataset includes 7 queries for each sample with binary labels. If the implicit exception handler did add a check type corresponding to the intent, then the label is a 1, and 0 otherwise.
Secondly, we evaluate on a dataset of ($M$, $S$) pairs for syntactic performance. 
Lastly, we evaluate on a dataset of ($M$, $O$) pairs for semantic performance.
For all datasets, we create a train/dev/test split at the project level of 81/6/6 to ensure that there is no project-level overlap between splits.

This amounts to a train/dev/test split of 23,930/2,621/4,255 for our generation datasets and a split of 167,790/18,347/29,785 for the intent dataset.  The dataset of intents is 7x larger as there is a data point for each intent type per sample. 


\subsubsection{Intent Query Model}
First, we evaluate the Intent Query Model in Table~\ref{tab:rq1-intent}. Additionally, we experimented with an encoder-only transformer model, CodeBERT~\cite{codebert}. 
We evaluate performance in terms of accuracy, precision, recall, and F1 score. Accuracy here is at the \textit{sample} level rather than query level. That is, a sample is correct iff $G_{intent}$ correctly predicted all 7 intent queries.


The models have comparable accuracy with CodeT5 performing with slightly higher F1. Although encoder-only BERT like models are better suited for a query/classification task,
CodeT5 has better performance as it is a larger model with nearly double the parameters (220M vs 125M). So, we select CodeT5 as our Intent Query Model architecture.


\begin{table}[t]
\resizebox{.45\textwidth}{!}{
{\small
	\begin{tabular}{ccccc}
	\toprule
		Intent Type & Accuracy & Precision & Recall & F1-Score \\
        \cmidrule(l){1-5}
		\textbf{CodeT5 Encoder}  & 84.93\%  & .88 & .91 & .89 \\
		CodeBERT &        84.83\%  & .86 & .91 & .88 \\
	 \bottomrule
	\end{tabular}
    }}
	\caption{RQ1: Evaluation of Intent Query Model.}
    \label{tab:rq1-intent}
\end{table}



\subsubsection{Precondition Generation Model}
\label{subsec:precond_gen_model_eval}
Next, we evaluate the generative CodeT5 model using the predicted intents from the Intent Query Model. We also evaluate the purely generative model without intent. 
We evaluate both approaches on syntactic and semantic metrics. For syntactic performance, we measure exact token-by-token match between predictions and labels.
For semantic metrics, we measure both suite-level and test-level accuracy.
by running the generated precondition against the test suite $O$ constructed during data collection.
For a prediction to be considered suite-level accurate, it must pass all tests in $O$. Test-level accuracy is a finer grained metric of accuracy. Since $O$ contains potentially multiple tests, test-level accuracy gives a measure of partial semantic correctness. 

Table~\ref{tab:rq1-gen} reports the performance for the overall dataset as well as the subset of samples with at least one intent. Samples without intent were non-crashing and have a precondition of ``{\small \texttt{return true;}}''. Because most MUTS are non-crashing, these samples heavily dominate our dataset comprising 50\%. We show this breakdown as the samples with intent are more challenging to predict. 
The CodeT5 model without intent performs comparably on the overall dataset with 75.53\% exact syntactic match. However, on the more challenging subset, the system with intent querying performs 6\% points better. Furthermore, the semantic evaluation shows an even greater discrepancy between the two approaches on the subset with at least one intent. At the suite-level, the system with intent querying performs over 15\% points higher. At the test-level, the gap rises to 20\% points. Thus, we find an end-to-end system with intent querying prior to generation improves the effectiveness of precondition generation over a purely generative system. 

Lastly, we note that both models produce preconditions which compile in the executable environment around 80\% of the time.


\begin{table*}[t]
\resizebox{.7\textwidth}{!}{
{\small
\begin{tabular}{c|cc|cc}
\toprule
                                       &     \multicolumn{2}{|c}{Overall}    & \multicolumn{2}{|c}{Samples with at least one Intent} \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5} 
                                       & Without Intent&  With Intent   & Without Intent   & With Intent \\
\midrule
               Exact Syntactic Match    & 75.53\%  & 76.92\%                            & 26.23\%     & 32.66\%    \\ 
               Suite-Level Semantic Match          & 81.6\%   & 82.16\% &                           42.41\%     & 58.70\% \\
               Test-Level  Semantic Match         & 78.5\%   & 81.00\% &                           62.13\%     & 82.02\% \\
\bottomrule
\end{tabular}
}}
\caption{RQ1: Evaluation of Generative Model.}
\label{tab:rq1-gen}
\end{table*}



%\begin{table*}[t]
%\resizebox{\textwidth}{!}{
%{\small
%\begin{tabular}{c|c|ccc|ccc|ccc|ccc|ccc}
%\toprule
%                     &              &         & Overall    &              &             & NPE       &            &             & Call       &             &             & Other       &           &             &Multiple Intents       &   \\ 
%\midrule
%                     &              & baseline & GT intent & End-To-End   & baseline    & GT intent & End-to-End  & baseline    & GT intent & End-to-End  & baseline    & GT intent & End-to-End  & baseline    & GT intent & End-to-End  \\
%\midrule
%                     & Accuracy     & 26.23\%   & 42.82\%   & 32.66\%    & 52.86\%     & 70.71\%   & 49.29\%      &  14.25\%    & 40.60\%   & 30.08\%     & 47.22\%     & 61.11\%   & 50\%       &   17.20\%    &  22.75\%  & 21.42\% \\ 
% Syntactic Metrics   & PPL          & ?         & ?         & ?          & ?           & ?         & ?            &  ?          & ?         & ?           & ?           & ?         & ?          &   ?          &   ?       & ? \\
%                     & BLEU         & ?         & ?         & ?          & ?           & ?         & ?            &  ?          & ?         & ?           & ?           & ?         & ?          &   ?          &    ?      & ?\\
%\midrule
%                    & Suite-level   & 42.42\%   & 45.18\%   & 61.39\%   & 66.42\%      & 72.69\%   & 63.10\%     &  32.81\%   & 50.78\%    & 38.80\%    & 47.22\%       & 65.71\%   & 62.86\%   &    32.25\%   &  37.40\%  & 34.42\% \\
% Semantic Metrics   & Test-level    & 62.13\%   & 59.80\%   & 87.23\%   & 75.97\%      & 84.81\%   & 77.09\%     &  60.51\%   & 68.04\%    & 65.20\%    & 50.59\%       & 41.18\%   & 87.65\%   &  57.19\%     &  56.33\% & 59.50\% \\
%                    & Compiles?     & 78.17\%   & 78.43\%   & 79.71\%   & 90.71\%      & 96.07\%   & 91.88\%     &  83.75\%  &  98.54\%    & 85.94\%    & 88.57\%       & 83.33\%   & 94.29\%   &  79.37\%     &  79.44\%  & 79.13\% \\
%\bottomrule
%\end{tabular}
%}}
%\caption{RQ1: Evaluation of Generative Model.}
%\label{tab:rq1-gen}
%\end{table*}

\noindent \begin{longfbox}
{\textbf{Result 1:} Our End-to-End system predicts 3,273 preconditions exactly syntactically equal to the label out of 4,255 samples (76.92\%). In comparison to a purely generation model without intent detection, it improves upon semantic accuracy by 20\% points.}
\end{longfbox}



\subsection{RQ2: Randoop Case Study} 
To answer RQ2, we run our end-to-end technique in conjunction with the randomized testing tool Randoop. Randoop employs API fuzzing to construct test prefixes that drive the given method to error revealing states. Because Randoop has no knowledge of a method's precondition, it uses a series of heuristics as described in Section~\ref{sec:setup}. The heuristics are intended to reduce FPs due to illegal inputs. However, they also mask true bugs in the process. In place of Randoop's heuristics, we propose using our predicted preconditions for each tested method. If the predicted precondition returns false, indicating that the input is illegal, we do not report the alarm.


\parheader{Bug Benchmark.} 
We evaluate real-world bug finding on the Defects4J~\cite{defects4j} benchmark and show the results in Table~\ref{tab:rq2-overall}. Defects4J is a benchmark of 835 bugs from 17 real world Java projects. Each bug is based on an error that was logged in the project's issue tracker and is based on a minimal patch. That is, Defects4J includes a series of snapshots of a project's evolution. For this case study, we randomly select three projects to evaluate on: Chart, Codec, and Lang. We run Randoop on each snapshot reporting total number of bugs found and average number of FPs per snapshot. We consider a bug ``found'' if there is at least one test which fails on the buggy version and passes on the fixed version. Lastly, we note that since our preconditions may modify state, we run them in a separate environment. %\TODO{I didn't actually do this. because it's rare that $S$ will modify state and it's a lot of work to implement I think... should we still mention it?}.  

An effective approach must reduce FPs without suppressing many TPs. As a comparison, we evaluate Randoop with its default heuristics settings. We also report Randoop's performance without any mechanism for precondition violation crash suppression. Lastly, we compare to TOGA which produces a binary exceptional oracle indicating that the input is legal or illegal.
Across all snapshots of the projects in our case study, our approach (denoted $S_\toolName{}$ reduces FPs by an average of 40\% while maintaining over 60\% of the TPs. In contrast, Randoop with heuristics reduces FPs significantly with nearly 0 FPs on average across snapshots. However, it also suppresses all TPs. Similarly, TOGA successfully reduces FPs by over 90\%, but also suppresses all TPs. Our approach provides a middle ground in which TPs are maintained at the sacrifice of a smaller reduction in FPs. \\ 

\begin{table*}[]
\centering
\resizebox{.7\textwidth}{!}{
\centering
    \begin{tabular}{c|c|cccc}
    \toprule
                    &                & Randoop without Heuristics    & $S_\toolName{}$ &     Randoop with Heuristics & Toga  \\
         \midrule
                    & Bugs Found     & 6                   & 5       & 0                   & 0   \\
         Chart      & Avg FPs        & 282                 & 131     & 0                   & 50   \\
                    %& FP per M      & 9                   & 4       & 0                   & 1.9    &? \\
         \midrule
                    & Bugs Found     & 2                   & 1       & 0                   & 0    \\
         Codec      & Avg FPs      & 507                 & 255     & 2                   & 2     \\
                    %& FP per M      & 56                  & 28      & .2                  & .2   & ? \\

        \midrule
                    & Bugs Found     & 4                   & 2       & 0                   & 0    \\ %& ?\\
         Lang       & Avg FPs       & 239                 & 164     & .2                  & 2    \\ %& ?\\
                    %& FP per M      & 27                  & 18      & .02                 & ?   & ? \\


         \bottomrule
    \end{tabular}
}
    \caption{RQ2: Randoop Case Study.}
    \label{tab:rq2-overall} 
\end{table*}





\noindent \begin{longfbox}
{\textbf{Result 2:} When hooked into Randoop, our generated preconditions reduce FPs by an average of 40\% while retaining 8 out of 12 bugs. In contrast to default Randoop and TOGA, our approach maintains a non-zero number of TPs while sacrificing a smaller reduction in FPs.}
\end{longfbox}

\subsection{RQ3: Robustness to Bugs}
The correctness of the MUT is unknown, and so the precondition generator should be able to infer
its precondition regardless of whether bugs exist in the MUT.
Moreover, the generator should not introduce bugs from the MUT into the precondition.

The Defects4J benchmark suite provides access to correct as well as buggy versions of methods.
Therefore, in order to answer RQ3, we run our end-to-end system for each buggy method in the Defects4J projects
\code{Chart}, \code{Codec}, and \code{Lang}, as well as on their corresponding correct methods, to obtain the
preconditions $S_\text{buggy}$ and $S_\text{correct}$.
A robust precondition generator should predict the same precondition for the correct as well as the buggy versions of
each method.
We therefore evaluate the robustness of the generator by applying the exact syntactic match metric described in
\autoref{subsec:precond_gen_model_eval} on $S_\text{buggy}$ and $S_\text{correct}$ obtained for each method.

\begin{table}[t]
\resizebox{.45\textwidth}{!}{
{\small
	\begin{tabular}{c|ccc}
	\toprule
		Project & Num Equal Predictions & Total Predictions & \% same \\
        \midrule
		Chart        & 32  & 44 & 72.73\% \\
		Codec        & 16  & 22 & 84.62\% \\
		Lang         & 59  & 88 & 67.05\% \\
        \midrule
		Total        & 107 & 154 & 69.48\% \\
	 \bottomrule
	\end{tabular}
    }}
	\caption{Whole Model Robustness to Bugs.}
    \label{tab:rq3-robustness}
\end{table}

\noindent \begin{longfbox}
{\textbf{Result 3:} Our End-To-End approach predicts the same precondition in the presence of a real world bug for 69.48\% of Defects4J's patched methods.}
\end{longfbox}


\subsection{Qualitative Analysis}
We consider two generated preconditions: one from Defects4J and one from our dataset's test split.

The MUT in Figure~\ref{fig:lang_33} is a member of the \texttt{Lang} Defects4J project. Our precondition successfully handles two classes of illegal inputs. The callee \texttt{deleteWhitespace} makes a call to \texttt{Character.isWhite} \texttt{space} which has undefined behavior on \textit{supplementary characters} whose code points are greater than U+FFFF. Our predicted precondition rejects illegal environments which crash the callee. Furthermore, our precondition captures the explicitly thrown \texttt{NullPointer} \texttt{Exception} as handling an illegal input.

Next we consider a MUT from our held out test set in Figure~\ref{fig:118423}. The MUT originated from the Apache POI project. Our generated precondition successfully handles both illegal input classes. The first, a \texttt{null} \texttt{data} array, and second, a \texttt{data} array of size zero.

%The MUT in Figure~\ref{fig:lang_33} is a member of the \texttt{Lang} Defects4J project. Our precondition successfully handles two classes of illegal inputs. The callee \texttt{deleteWhitespace} makes a call to \texttt{Character.isWhitespace} which has undefined behavior on \textit{supplementary characters} whose code points are greater than U+FFFF. Our predicted precondition rejects illegal environments which crash the callee. Furthermore, our precondition captures the explicitly thrown \texttt{NullPointerException} as handling an illegal input.


\begin{figure} % [hb]
    \begin{subfigure}[b]{0.49\linewidth}
    \lstset{style=mystyle, xleftmargin=.0\textwidth, xrightmargin=0.2\textwidth, linewidth=0.2\linewidth}
    \lstinputlisting[linewidth=9.2cm]{./examples/Lang_33_.java}
    \caption{MUT}
    \label{fig:lang_33_mut}
    \end{subfigure}

    \begin{subfigure}[b]{0.49\linewidth}
    \lstset{style=mystyle, xleftmargin=.0\textwidth, xrightmargin=0.2\textwidth, linewidth=0.2\linewidth}
    \lstinputlisting[linewidth=9.2cm]{./examples/Lang_33_pre.java}
    \caption{Precondition}
    \label{fig:lang_33_pre}
    \end{subfigure}

   \caption{MUT and its corresponding precondition.}
    \label{fig:lang_33}
\end{figure}


\begin{figure} % [hb]
    \begin{subfigure}[b]{0.24\linewidth}
    \lstset{style=mystyle, xleftmargin=.0\textwidth, xrightmargin=0.0\textwidth, linewidth=0.2\linewidth}
    \lstinputlisting[linewidth=5.5cm]{./examples/MUT118423.java}
    \label{fig:118423_mut}
    \end{subfigure}

    \begin{subfigure}[b]{0.24\linewidth}
    \lstset{style=mystyle, xleftmargin=.0\textwidth, xrightmargin=0.0\textwidth, linewidth=0.2\linewidth}
    \lstinputlisting[linewidth=5.5cm]{./examples/Label118423.java}
    \label{fig:118423_pre}
    \end{subfigure}

   \caption{MUT and its corresponding precondition.}
    \label{fig:118423}
\end{figure}

\subsection{Error Analysis} 
We perform an error analysis of our system's precondition generation by intent/crash type. The call intent type performs the worst.
To better understand this, we perform a manual study of 25 preconditions with call intent that our end to end model incorrectly predicts. In 11 of the cases, our intent model selected the wrong intent (see Table~\ref{tab:rq1-intent}). In 7 of the cases, our model correctly predicted a call intent, but the generative model surrounded an incorrect call in a try catch. In the remaining cases, the true precondition contained multiple calls in try-catch blocks, but our model only selected one.
An improved intent model, and improved call generative modeling, may be achieved with carefully selected context as input. The signatures or body's of callees may be useful in selecting the correct call to wrap in a try-catch. Lastly, a mechanism to select which the number of calls as part of the intent label may be beneficial.

\subsection{Threats to Validity}
Bias in Randoop's performance is a potential threat to validity. Our evaluation of RQ2 shows that the preconditions generated by our approach (\toolName{})
can suppress FPs but cannot discover new bugs. As a result, we do not evaluate our approach on bugs missed by Randoop.


==> old_submission/old_6_limitations.tex <==
\section{Limitations}
\label{sec:limitations}

Our training dataset is comprised exclusively of correct code. This is a limitation of our system, which sees buggy code only at test time. 
A model would potentially benefit from data augmentation through injecting faults to better infer preconditions in the presence of a bug.
While this is a limitation, we found that our system is robust to bugs in almost 70\% of the patched methods, indicating our model's ability to generalize.

Furthermore, our training dataset distribution is not even across crash types. The top-3 most common crash types comprise almost 99\% of the dataset, with 4 other crash types only making up 1\%.
This is a limitation of our model's performance on the less seen crash types. Data augmentation using synthetically generated samples may address this.
Although our dataset is skewed toward some crash types, we also observed a similar bias in Defects4J projects, indicating that the bias may be preferable.

Another limitation of our approach is that the intent model does not predict the number of checks to add. For example, an intent of \texttt{CALL} may represent wrapping a single call in a try-catch or multiple. This is a task which we leave to the generative model.



==> old_submission/old_7_conclusions.tex <==
\section{Conclusion}
\label{sec:conclusion}

This paper presents precondition inference as a code generation task. It provides the first large scale dataset of (method, precondition) pairs. It also provides a dataset of test suites along with executable environments to perform semantic evaluation of generated preconditions. Furthermore, it proposes a neural language model approach with intent detection and prompt based learning. Applied to a bug finding task, our approach can generate preconditions to reduce Randoop FPs by 40\% on average while retaining most TPs.



==> old_submission/old_intro.tex <==
\section{Introduction}
\label{sec:introduction}
Program specifications are an oracle of correct program behavior with applications in verification~\cite{JML,Z,Spec_sharp}, program comprehension, and dyanmic~\cite{Korat} and static bug finding~\cite{esc-java}. Although beneficial, program specifications are rarely written in practice~\cite{c2s}. Instead, intent is convyed through docstring commments, identifier names and program context, or entirely omitted. In this paper, we investigate specification inference from these sources. 

As an application, we investigate precondition inference for dynamic bug finding. Dynamic bug finding tools execute a unit under test with many different input states attempting to find a state which crashes the unit~\cite{Randoop, AFL, Korat}. The crashes are typically reported to the developer as bugs. However, from a developer's perspective, a crash does not necessarily indicate a bug. Often, a crash is intended. When an input condition (\textit{precondition}), is not satisfied prior to executing the unit, a common strategy is to raise an exception and crash the program. A crash caused by a violated precondition is not a bug in the method under test, but instead a bug in the caller. As such, it is not helpful for precondition violations created by the testing tool to be reported to the developer. Unfortunately, most units have an implicit precondition, but they are rarely formally written in practice. Automated testing tools resort to heuristics to decide if a crash was a precondition violation or a true fault. If automated testing tools had knowledge of a method's precondition, they could  suppress precondition violating crashes (false positives) without masking true bugs (false negatives).

The dynamic bug finding tool Randoop fuzzes units by constructing sequences of API calls that drive the unit to interesting states. If a preecondition is not specificed, Randoop relies on hueriestics to decide if a craash is inteended. In the following example, we consider any crash a bug.
The figure shows a \texttt{Stack} class with a bug in \texttt{push}. For this example we consider all other methods correct wrt to the intent. 

\begin{figure}[hb]
    \lstset{style=mystyle, xleftmargin=.0\textwidth, xrightmargin=0.0\textwidth, linewidth=0.95\linewidth}
    \lstinputlisting[linewidth=8cm]{./examples/Stack.java}
    \caption{Stack class containing a bug.}
    \label{fig:pop_ex}
\end{figure}

The \texttt{pop} method has an explicit precondition: the stack must not be empty at it's entry. The constructor \texttt{Stack}

Running Randoop for 5 seconds results in 136 crashing tests found. Of the 136 crashes, only 32 (24\%) were related to the precondition. All 101 other crashes (76\%) were precondition violations (false positives). The majority of crashes were due to a precondition violation of pop. There were also 3 precondition violations of the constructor \texttt{Stack}. Here, the precondition is implicit: \texttt{maxSize >= 0}. For a developer inspecting these alarms, 104 false alarms may be problematic.

If randoop had acccess to the following preconditions it could suppress the false positives and only report true bug crashes to the developer. 
\begin{figure}[hb]
    \begin{subfigure}[b]{0.3\linewidth}
    \lstset{style=mystyle, xleftmargin=.0\textwidth, xrightmargin=0.2\textwidth, linewidth=0.2\linewidth}
    \lstinputlisting[linewidth=4.2cm]{./examples/Pre_Pop.java}
    \label{fig:pop_pre}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\linewidth}
    \lstset{style=mystyle, xleftmargin=.1\textwidth, xrightmargin=0.0\textwidth, linewidth=0.2\linewidth}
    \lstinputlisting[linewidth=4.5cm]{./examples/Pre_Stack.java}
    \label{fig:pre_stack}
    \end{subfigure}

   \caption{Preconditions of the \texttt{Pop} method and the \texttt{Stack} constructor }

\end{figure}


There 
Previous approaches don't work becaause ....aA


We formulate preconditiono infeerence as an executable method.


\textit{Contributions.} In summary, this paper:
\begin{enumerate}
\item Formulates precondition inference as a program generation task
\item Introduces a language-model based approach to generate executable exceptional preconditions. 
\item Presents a dataset of (method, precondition) pairs included in our open source release.
\item Presents an executable semantic evalutaion metric for code generation.
\item Performs an evaluation on precondition inference. We demonstrate that our approach reduces false positives by YYY.
\end{enumerate}


==> old_submission/old_overview.tex <==
\section{Illustrative Overview}

In this section, we motivate and illustrate our approach for inferring preconditions with an application to automated test generation
and bug finding.
Consider a simplified version of the \code{createNumber} method from the \code{Lang} project in the Defects4J benchmark.
The simplified method \code{createNumber} takes a character \texttt{a} and attempts to return an integer representation of \texttt{a}.
This method is a partial function where non-digit characters are considered illegal inputs. 
%\TODO{Should I bring up the bug here? No. probably not.}
This version of \code{createNumber} contains a bug on the upper bound of ASCII digits. 
The developer made an off by one error in the if condition. The integer literal ‘56’ should be ‘57’ since ASCII values 48-57 correspond to digits.

%The correct version is shown in  \autoref{fig:correct_example}, while the buggy version is shown in \autoref{fig:buggy_example}.
%The bug results from passing \code{colKey} as the argument to \code{rowData.getObject} in line 24, without performing the necessary checks
%highlighted in green in \autoref{fig:correct_example}.
% \autoref{fig:correct_example} shows the \emph{correct} version of the \code{getObject} function, while
% \autoref{fig:buggy_example} shows the \emph{buggy} version of the same.
% The bug is in line 5 of \autoref{fig:buggy_example}, where there is a missing, but required, null check for
% object \code{r}, defined on line 3. Due to this bug, \autoref{fig:buggy_example} might unintentionally throw a
% \code{NullPointerException} when executed.

% randoop

Running an automated test generation tool such as \randoop{} on the buggy version of \texttt{createNumber} produces over 700 crashing test cases.
However, all of them are false alarms. Figure \autoref{fig:false_positive} shows a test case that exhibits such a false alarm.
The input \texttt{'U'} is not a legal input to \texttt{createNumber} as it is not a digit. Presenting such alarms to the developer are
not helpful as it is expected behavior. On the other hand, figure \autoref{fig:true_positive} shows a test case revealing the bug. 
This test case, which ideally would be the only alarm presented by the developer, was not found by Randoop. \TODO{maybe don't say that randoop didn't even find it... Pretend it did...}

%In order to reduce such false alarms, \randoop{} provides a set of heuristics that capture common patterns of false alarms,
\randoop{} provides a set of heuristics to reduce such false alarms. The heuristics capture common patterns of false alarms,
such as a \code{NullPointerException} thrown on a \code{null} argument of the method being tested.
However, these heuristics are inherently noisy: at the expense of reducing large classes of false alarms, they
also suppress real bugs. \TODO{point to the figure from the Randoop documentation?}
% , and thereby lack knowledge of the semantics of the method being tested.

\randoop's inaccurate behavior in classifying legal from illegal environments can be attributed to its lack of knowledge of the developer intent.
% \autoref{fig:precondition_example} shows the precondition of the \code{getObject} method.
% It is a method which takes as input the environment, and returns \true{} if and only if it is legal.
% While \randoop{} allows the user to provide such specifications, however, they are seldom provided in practice.
% Therefore, a number of approaches have been proposed to automatically infer them.
\randoop{}, therefore, allows the user to provide specifications to address its inaccuracies.
However, such specifications are tedious to formulate, and as such are seldom provided in practice.

To address the challenge of manually writing specifications, there has been much work in precondition generation and discovery. 
Most prior works on generating preconditions have focused on generating a declarative symbolic specification of the method under test (MUT), 
{\it assuming} the method does not contain any bugs. 
%Most existing approaches analyze the method under test to infer specifications in the form of a predicate which
%classifies crashing behaviors from non-crashing ones.
For example, specification discovery tools generate a logical specification from runs of a program. 
Invariant discovery tools like Daikon~\cite{daikon} report logical invariants which are true across all program executions. 
For example, given a stack class, across all runs to the program, the capacity is always >= 0. 
Daikon has logical numeric templates like this and they find a predicate which satisfies all of the observed runs.
Such an approach has many limitations, one being that they assume the method under test is correct.
An invariant discovery tool would consider \code{a = 57} to be a bad or crashing run. 
Thus, the predicate it creates would not be satisfied by \code{a = 57}, and the predicate would propagate the bug: \code{a >= 48 \&\& a <= 56}. 
Such a predicate would not be useful in the bug finding scenario as \code{a == 57} would be classified as a precondition violation. 
For this reason, invariant discovery tools cannot be used at inference time in the bug finding scenario. 

%Even then, these approaches are intractable due to the undecidable nature of classifying program behaviors.
%For example, the precondition inferred for \code{getObject}
%would declare an environment illegal if it violated the following condition: \code{rowKey == null || colKey == null}.
%However, predicates cannot fully represent the intent of the method under test, since they are unable to capture rich and stateful
%patterns.

%\TODO{talk here about why we make it executable...maybe move some of the content from the introduction /datasest section here}.
%We therefore propose to represent preconditions as executable methods, as shown in \autoref{fig:precondition_example}.
%Such preconditions are methods which take as input the environment, and return true if and only if it is legal.
%Since they are expressed as code, they allow for performing checks on deeper semantic patterns of the method, such as over
%the post state of the callees within \code{getObject}.
%They can also capture patterns that may be nested within several functions, as shown in the precondition in
%\autoref{fig:pre_mut_nested_call}, which can declare an environment to be illegal if \code{next(1)} throws an exception.
%Finally, they can also be used in unit tests such as the ones shown in \autoref{fig:tests} to perform checks before
%calling the method itself.
%For example, to check the legality of the input to \code{getObject} in \autoref{fig:false_positive},
%the check ``\code{if (getObject\_pre(100, -1))}'' can be inserted such that \code{getObject} is called only if
%the check evaluates to true.

Because Randoop requires manual input to specify developer intent and current approaches for precondition generation are not sufficient, 
we formulate the precondition inference problem as a learning task. 

Large language models such as CodeBERT \cite{codebert}, Codex~\cite{Codex} and CodeT5 \cite{CodeT5} that are pretrained over code have shown promise in code generation tasks.
Moreover, they have also shown an ability to reason over the semantics of methods. Machine learning is good for learning developer intent through syntactic and natural language signals\TODO{cite bassically all my papers}.

%We therefore propose to use such models as the code generator to address the aforementioned challenges.
As these models are generative, AND BECAUSE PRECONDITIONS EXIST AS INTERMINGLED COMPUTATION, 
this leads us to formulate the precondition inference problem as a code generation problem.

%This formulation introduces a set of challenges.
%First, the generator must be able to infer the intent of the method's designer in order to generate the precondition.
%This is challenging, since the intent is often implicit within the method, and may be dependent on computations
%%performed in the method.
%The generator must, therefore, be able to intelligently discern the checks and computations within the method
%that are indicative of the intent.
%The second challenge is that the correctness of the method is not known.
%As a result, the generator must avoid introducing bugs that may appear within the method into the generated precondition.

%cite

In order to train and evaluate the generator model, a dataset of methods and their respective preconditions is required.
We restrict the curation of this dataset to a set of well-known, high-quality, and extensively tested Java projects,
which allows us to assume the methods to be correct in order to obtain their preconditions.
Even though the aforementioned approaches to precondition inference work with the same assumption, they are not
able to effectively scale to the size of the dataset required for training the generator model.
To address this challenge, we propose a technique that can extract the preconditions for the methods
in a scalable manner.


\begin{figure}[]
    \centering
    \begin{subfigure}[b]{1.0\linewidth}
        \centering
        \lstset{style=mystyle, xleftmargin=.0\textwidth, xrightmargin=0.0\textwidth, linewidth=0.2\linewidth, numbers=left, frame=none, breaklines=false}
        \lstinputlisting[]{./examples/false_positive.java}
        \caption{A test reporting a false positive.}
        \label{fig:false_positive}
    \end{subfigure}
     
    \begin{subfigure}[b]{1.0\linewidth}
        \centering
        \lstset{style=mystyle, xleftmargin=.0\textwidth, xrightmargin=0.0\textwidth, linewidth=0.2\linewidth, numbers=left, frame=none, breaklines=false}
        \lstinputlisting[]{./examples/true_positive.java}
        \caption{A test reporting a true positive.}
        \label{fig:true_positive}
    \end{subfigure}

   \caption{An example of two tests over \code{createNumber} reporting a false positive and a true positive respectively.}
    \label{fig:tests}
\end{figure}


%\begin{figure} % [hb]
%    \centering
%    \lstset{style=mystyle, xleftmargin=.0\textwidth, xrightmargin=0.0\textwidth, linewidth=0.2\linewidth, numbers=left, frame=none}
%    \lstinputlisting[linewidth=9cm]{./examples/pre_example.java}
%    \caption{The precondition for the \code{getObject} function.}
%    \label{fig:precondition_example}
%\end{figure}


\begin{figure} % [hb]
	\centering
    \begin{subfigure}{0.3\linewidth}
    \lstset{style=mystyle, xleftmargin=.0\textwidth, xrightmargin=0.2\textwidth, linewidth=0.2\linewidth}
    \lstinputlisting[linewidth=4.2cm]{./examples/OperatorName.java}
    \caption{MUT}
    \label{fig:mut_nested_call}
    \end{subfigure}
    \begin{subfigure}{0.3\linewidth}
    \lstset{style=mystyle, xleftmargin=.1\textwidth, xrightmargin=0.0\textwidth, linewidth=0.2\linewidth}
    \lstinputlisting[linewidth=4.5cm]{./examples/Pre_OperatorName.java}
	\vspace{0.17in}
    \caption{Precondition}
    \label{fig:pre_mut_nested_call}
    \end{subfigure}

   \caption{MUT and its corresponding precondition, where the MUT has a nested call.}
    \label{fig:mut_example}
\end{figure}




% Assume method is correct, cannot capture complex patterns due to the undecidable nature of classifying

% Automatically inferring such a precondition from the method under test poses several challenges.

% In order to reduce the number of these false positives -- heuristic flags -- turning them on suppresses most of these false positives
% but also suppresses the bug itself -- preconditions needed to balance this out

% \randoop{} provides a set of heuristic flags, which can be specified in order to suppress false positives.
% Without any of these flags, \randoop{} will find the bug in line 5, but will also produce \textbf{84} false positives.
% On the other hand, turning these flags on results in \textbf{0} false positives, but also suppresses the actual bug,
% resulting in a false negative.

% The heuristics that these flags represent are very rigid and too coarse to suppress false positives without
% suppressing the bug itself.
% A more fine-grained alternative to using such heuristic flags is to write the actual preconditions themselves and pass them to \randoop{}.
% One approach to writing preconditions is to do so manually.
% However, this tends to be difficult, since methods like \code{getObject} are oftentimes large and complex, and discerning
% the implicit intent of these methods tends to be challenging.

% \TODO{Find examples for these??}
% These challenges have resulted in several automated tools that try and synthesize the preconditions from the method.
% For example, purely symbolic tools like \TODO{Daikon, JIST \cite{jist}} use engineered heuristics % ESCJava?
% to infer preconditions from the definition of the method itself.
% However, these heuristics often address only a subset of the vocabulary of the entire language, and therefore tend to
% not work with complex methods.

% On the other hand, data-driven tools %that rely on a set of test executions to infer the precondition
% like \TODO{SnuggleBug \cite{snugglebug}, PreGen \cite{data-driven}} overcome this obstacle
% by inferring preconditions from a set of features obtained by the dynamic behavior of the method.
% However, such tools rely on assuming that the method is correct, and inferred preoconditions from incorrect methods
% may treat the buggy behaviors of those methods as being intended behavior.
% \TODO{Do we need examples of preconditions generated for the buggy version by such tools? Otherwise we are just repeating
% the introduction}

% In contrast, our approach of treating precondition inference as a code generation task allows us to work with such complex
% methods while being robust to bugs that may be present in these methods.
% The precondition inferred by our approach from \autoref{fig:buggy_example} is shown in \autoref{fig:precondition_example}.
% This precondition results in \textbf{64} false positives, suppressing \textbf{20} of those reported by heuristic-free \randoop.
% In contrast to \randoop{} with the heuristic flags, our approach does not suppress the actual bug.


% public Object getObject(Comparable rowKey, Comparable columnKey) {
%         if (rowKey == null) {
%             throw new IllegalArgumentException("Null 'rowKey' argument.");
%         }
%         if (columnKey == null) {
%             throw new IllegalArgumentException("Null 'columnKey' argument.");
%         }
%         int row = this.rowKeys.indexOf(rowKey);
%         if (row < 0) {
%             throw new UnknownKeyException("Row key (" + rowKey 
%                     + ") not recognised.");
%         }
%         int column = this.columnKeys.indexOf(columnKey);
%         if (column < 0) {
%             throw new UnknownKeyException("Column key (" + columnKey 
%                     + ") not recognised.");
%         }
%         if (row >= 0) {
%         KeyedObjects rowData = (KeyedObjects) this.rows.get(row);    xxxxxxx
%             return rowData.getObject(columnKey);
%         }
%         else {
%             return null;
%         }
%     }


% public Object getObject(Comparable rowKey, Comparable columnKey) {
%         if (rowKey == null) {
%             throw new IllegalArgumentException("Null 'rowKey' argument.");
%         }
%         if (columnKey == null) {
%             throw new IllegalArgumentException("Null 'columnKey' argument.");
%         }
%         int row = this.rowKeys.indexOf(rowKey);
%         if (row < 0) {
%             throw new UnknownKeyException("Row key (" + rowKey 
%                     + ") not recognised.");
%         }
%         int column = this.columnKeys.indexOf(columnKey);
%         if (column < 0) {
%             throw new UnknownKeyException("Column key (" + columnKey 
%                     + ") not recognised.");
%         }
%         KeyedObjects rowData = (KeyedObjects) this.rows.get(row);    xxxxxx
%         int index = rowData.getIndex(columnKey);
%         if (index >= 0) {
%             return rowData.getObject(index);
%         }
%         else {
%             return null;
%         }
%     }

% precondition(...) {	
%         if (rowKey == null) {
%             return false;
%         }
%         if (columnKey == null) {
%             return false;
%         }
%         int row = this.rowKeys.indexOf(rowKey);
%         if (row < 0) {
%             return false;
%         }
%         int column = this.columnKeys.indexOf(columnKey);
%         if (column < 0) {
%             return false;
%         }
% 	reutrn true;
% }

% public boolean getObject_precondition(Comparable rowKey, Comparable columnKey) {
%         int row;
%         try {
%             row = this.rowKeys.indexOf(rowKey);
%         } catch (Exception e) {
%             return true;
%         }
%         if (columnKey == null)
%             return true;
%         try {
%             this.columnKeys.indexOf(columnKey);
%         } catch (Exception e) {
%             return true;
%         }
%         return false;
%     }


% SCRIPT

% testing tool on the buggy version and it produces XXX crashes.
% Vast majority of them are false positives.


==> old_submission/old_problem_setup.tex <==
\section{Problem Setup}
\label{sec:setup}


\begin{figure} % [hb]
    \begin{subfigure}[b]{0.3\linewidth}
    \lstset{style=mystyle, xleftmargin=.0\textwidth, xrightmargin=0.2\textwidth, linewidth=0.2\linewidth}
    \lstinputlisting[linewidth=4.2cm]{./examples/OperatorName.java}
    \label{fig:pop_pre_setup}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\linewidth}
    \lstset{style=mystyle, xleftmargin=.1\textwidth, xrightmargin=0.0\textwidth, linewidth=0.2\linewidth}
    \lstinputlisting[linewidth=4.5cm]{./examples/Pre_OperatorName.java}
    \label{fig:pre_stack_setup}
    \end{subfigure}

   \caption{MUT and its corresponding precondition}

\end{figure}

% Problem Statement:
% A exception oracle is a function C : Method M -> (Input I -> Bool).

% Let C_ideal be the ideal (and unrealizable) bug classifier.
% We seek to learn C ~ C_ideal.

% Notes:
% 1. We know C_ideal(M*, I) = No Bug for known correct method M* and all I.
% 2. We know C_ideal(M, I) for certain M, I such as for Defects4J suite.
%    So we can measure false alarms and missed bugs.

% There are many different ways to construct C.

% // Baseline 1:
% C_randoop = lambda M, I .
%    ... // describe Randoop's heuristic here (copied from its manual)

% // Baseline 2:
% C_toga = lambda M, I .
%    ... // see ICSE'22 paper

% // Baseline 3:
% Construct a G : Method -> Spec using predefined NL+PL heuristics (no ML).
% C_jdoctor = lambda M, I. check(M, G(M), I)


In order to formulate precondition inference as a code generation problem, we first define exception oracles,
which are used to distinguish legal inputs or environments from illegal ones.
Let $\domain{P}$ denote the set of all executable methods,
and $\domain{E}$ denote the set of all program environments. An exception oracle can then be defined
as the function $C : \domain{P}, \domain{E} \rightarrow \code{Bool}$ which returns \true{} for illegal
inputs and \false{} for expected ones.

Let $\cIdeal$ denote the ideal precondition. Such an oracle will exhibit the following behavior
for a particular correct method $M* \in \domain{P}$:
$$
\forall I \in \domain{E}, \cIdeal{}(M*, I) = \false
$$

Additionally, for any method $M \in \domain{P}$,
% certain environments can be considered to be legal,
% such that they are compliant with the intent of $M$, while the rest that violate the intent of $M$
% can be considered to be illegal. In such cases, any crash on $M$ with some legal environment is
% considered to indicate a bug, while any crash with an illegal environment is indicative of an unexpected
% crash. Let the set of legal environments for $M$ be $\domain{E}_{legal}$,
% and that of illegal environments be $\domain{E}_{illegal}$. Then
$\cIdeal$ exhibits the following behavior:
$$
    \forall I \in \domain{E}, \cIdeal{}(M, I) =
        \begin{cases}
            \true & \text{ if I is an illegal input to M} \\
            \false & \text{ otherwise}
        \end{cases}
$$

\TODO{Add note about knowing $\cIdeal$ for the Defects4J dataset}

Since $\cIdeal$ cannot be realized, an assortment of definitions for $C$ exist across different
automated testing tools, with varying effectiveness. For instance, the exception oracle used
by \randoop{} is defined via engineered heuristics: \TODO{Add definition}

\toga{} uses a binary classification model as its exception oracle: \TODO{add definition}

\jdoc{} uses predefined natural language heuristics to define a function $H$ \TODO{Add definition}.

We propose to define an exception oracle function by synthesizing executable preconditions.
Let the set $\domain{S} \subseteq \domain{P}$ denote the set of all the executable preconditions.
We construct a function $G : \domain{P} \rightarrow \domain{S}$ to synthesize the minimal executable
precondition given some $M \in \domain{P}$.
We can then define the exception oracle as follows in terms of \code{check} as detailed in Algorithm
\ref{alg:check}:
$$
\forall I \in \domain{E}, \cOurs(M, I) = \code{check}(M, G(M), I).
$$
Our goal, therefore, is to learn the function $G$ such that $\cOurs$ can approximate $\cIdeal$ as
closely as possible.
The definition of $G$ can be learned by training a
machine learning model over a dataset of pairs of $(M*, S) \in \domain{P} \times \domain{E}$, where
$M*$ is a \emph{correct} method, and $S$ is its minimal executable precondition.

% ======================================================================
%     check : (Method M, Spec S, Input I) -> Bool
%         If M(I) throws an exception
%            return No Bug
%         else
%            if S(I) == True
%               return No Bug
%            else
%               return Bug
% ======================================================================

\input{algorithms/check.tex}

This effectively represents the problem of defining the exception oracle as a code generation problem.
Doing so has several advantages over alternate approaches, since it is: % previous approaches, since \toolName{} is:
\begin{enumerate}
    \item \textbf{Interpretable.}
        The setup aims to synthesize a minimal executable precondition for a method. The minimality
        allows for the precondition to be easily interpretable, since a developer can examine the generated
        code to ensure that the precondition is correct. Moreover, the developer can even edit the precondition
        in case the precondition does not fully express the intent of the method, and commit it for use in further
        testing. \TODO{why is an executable method easier to edit than a predicate?. Idk if we should keep this.}
    \item \textbf{Expressive.}
        The minimality of the generated precondition also allows for it to be easily documentable. A state-of-the-art
        code summarization tool can use the precondition to synthesize natural language documentation that can
        effectively describe the method its expected behavior.
    \item \textbf{Portable.}
        The executability of the generated preconditions ensures that they are portable, meaning that they can
        be used with any testing tool by integrating the preconditions into the test drivers generated for that
        method. On the other hand, tools like \toga{} are trained over environments generated by specific
        testing tools that cannot be generalized to other tools, and porting the exception oracle used by
        Randoop for use in other tools would require heavy engineering efforts.
\end{enumerate}

In order to realize \toolName{}, we must address two significant challenges:
\begin{enumerate}
    \item \textbf{Generating the Dataset.}
        This is hard because of a bunch of reasons.
        In accordance to our insight, we can obtain the dataset from a suite of trusted projects.
        Talk about Dtrain \ $\widetilde{}$ \ Dtest.
    \item \textbf{Learning the precondition synthesis function $G$.}
        This is hard because of a whole bunch of other reasons, like a bajillion reasons.
        Summarize the insight of boosting generation with intents.
        Some challenges, including how to evaluate $G$ and the metrics.
\end{enumerate}

% ======================================================================
%     Input: Corpus of correct methods D = { M1*, ..., Mk* }
%     Output: { <M*, S> | S is the exception precondition of M* in D }
%     Algorithm 1:
%     for each M* in D: // simplified
%        (1) Run EvoSuite to generate a set of inputs I1, ..., In
%        (2) Run Perses to find a minimal boolean program S from M*
%            such that S(I) = true iff M*(I) crashes
%        (3) output <M*, S>
% ======================================================================



% =========================================================================
% // Our Approach:
% Construct a G : Method -> Spec from a dataset D_train of (M*, S) pairs.
% C_ours = lambda M, I . check(M, G(M), I)

% // Thought experiment: What if S = M?

% Strengths of our approach over previous approaches:
% - Interpretable: human can change it if it is incorrect, and commit the spec for future regression tests.
% - Documentation: take the spec and produce natural language documentation
% - Portable: works with any testing tool.  E.g. C_toga is trained on I's coming from specific testing tool.
%   - Note: this relies on Spec being executable!

% There are two challenges to realize our approach:

% Challenge 1 (Dataset Generation): How to construct D_train?
%    Explain in words why this is hard.
%    Our insight: Note (1) above.
%    Now describe Algorithm 1.
%    Need to explain informally why D_train ~ D_test

% Challenge 2 (Learning): How to learn our G?
%    Explain in words why this is hard (generation of an executable and correct spec is hard!)
%    Our insight: intent + generation
%    Explain the model.
%    How do we know we learnt a good G?
%    Describe our evaluation metric based on Note (2).
% ======================================================================



